VoMP: Predicting Volumetric Mechanical Property Fields

Physical simulation relies on spatially-varying mechanical properties, often laboriously hand-crafted. VoMP is a feed-forward method trained to predict Young's modulus ($E$), Poisson's ratio ($\nu$), and density ($\rho$) throughout the volume of 3D objects, in any representation that can be rendered and voxelized. VoMP aggregates per-voxel multi-view features and passes them to our trained Geometry Transformer to predict per-voxel material latent codes. These latents reside on a manifold of physically plausible materials, which we learn from a real-world dataset, guaranteeing the validity of decoded per-voxel materials. To obtain object-level training data, we propose an annotation pipeline combining knowledge from segmented 3D datasets, material databases, and a vision-language model, along with a new benchmark. Experiments show that VoMP estimates accurate volumetric properties, far outperforming prior art in accuracy and speed.

==> fig/arch.tex <==
\begin{figure}
    \centering
    \includegraphics[width=.4\linewidth]{example-image-b}
    \caption{\textbf{Network Architecture.} We show the network architecture of MatVAE and Geometry Transformer.}
    \label{fig:arch}
\end{figure}

==> fig/comapre_fields.tex <==
\begin{figure*}
    \centering
    \includegraphics{assets/fields.pdf}
    \caption{\textbf{Mechanical Property Fields.} We compare mechanical property fields estimated by \acronym\ and the baselines~\cite{zhai2024physicalpropertyunderstandinglanguageembedded, shuai2025pugszeroshotphysicalunderstanding, lin2025phys4dgenphysicscompliant4dgeneration}. We show the color coded fields and slice planes through the fields. We observe significnatly more accurate volumetric property fields than the baselines (\video{00:00}).}
    \label{fig:comparefields}
\end{figure*}

==> fig/ficus_container.tex <==
\begin{figure}[tb]
    \centering
    \setlength{\tabcolsep}{0pt}
    \includegraphics{assets/ficus_container.pdf}
    \bigarrow{time}
    \caption{\textbf{Simulating Dropping Ficuses.} We simulate 65 3D Gaussian Splats with properties estimated by \acronym\ falling into a container. (\video{00:00})}
    \label{fig:ficus_container}
\end{figure}

==> fig/fig_teaser.tex <==
% \begin{figure*}
% \centering
%   \includegraphics[width=0.98\textwidth]{img/tmp_teaser.png}
%   \caption{Take a few scanned objects, and arrange them in a scene and then run some rigid robot in the scene. }
%   \label{fig:teaser}
% \end{figure*}
\twocolumn[{%
  \renewcommand\twocolumn[1][]{#1}%
  \maketitle
  \begin{center}
    \includegraphics[width=\linewidth]{assets/teaser.pdf}%
    \captionof{figure}{\textbf{\acronym} brings geometry to life by taking in mesh, 3D Gaussian Splat, SDF, NeRF, and more 
    % \masha{adjust wording to make clear this list is not exhaustive}
    and estimates volumetric, physically accurate, and dense mechanical property fields of Young's Modulus, Poisson's Ratio, and Density (\textit{right}). These mechanical property fields can be used within an accurate simulator to produce realistic deformable simulations. We show an elastodynamic simulation (\textit{left}) of a dozer going through a forest of 100 ficuses (gaussian splats) using the estimated mechanical property fields (\video{00:00}).}
    % \masha{Really cool figure! What's with the inconsistent colors for ficus/dozer? Ficus should also be labeled as Splat, but I would suggest labeling dozer as splat/mesh, just to communicate it doesn't matter.}}
    \label{fig:teaser}
  \end{center}
  %\vspace{-0.8\baselineskip}
}]

==> fig/iclr/comapre_fields.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{assets/fields.pdf}
    \caption{\textbf{Mechanical Property Fields.} We compare mechanical property fields estimated by \acronym\ and the baselines~\cite{zhai2024physicalpropertyunderstandinglanguageembedded, shuai2025pugszeroshotphysicalunderstanding, lin2025phys4dgenphysicscompliant4dgeneration}. We show the color coded fields and slice planes through the fields. We observe significnatly more accurate volumetric property fields than the baselines (\video{00:00}).}
    \label{fig:comparefields}
    \vspace{-1em}
\end{figure*}

==> fig/iclr/matvae_grid.tex <==
\newcolumntype{P}{>{\centering\arraybackslash}m{1.5cm}}
\newcolumntype{C}{>{\centering\arraybackslash}m{\cellsize}}

\begin{wrapfigure}{l}{0.5\textwidth}
    \vspace{-2em}
    \centering
    \setlength{\tabcolsep}{0pt}%
    \renewcommand{\arraystretch}{0}%
    \newlength{\arrowcol}
    \setlength{\arrowcol}{0.08\columnwidth} % width of the arrow column
    \newlength{\cellsize}
    \setlength{\cellsize}{\dimexpr(\columnwidth-\arrowcol)/5\relax}
    \newcommand{\squarecell}[2]{%
      \cellcolor{#1}{%
        \color{white}\parbox[c][\cellsize][c]{\cellsize}{\centering #2}%
      }%
    }
    \resizebox{0.5\textwidth}{!}{%
    \begin{tabular}{c c c c c c}
    % Top header row
    & \multicolumn{5}{c}{\bigarrowleftright{Latent Dimension 1}} \\
    % Left multirow rotated label + data rows
    \multirow{5}{*}{\rotatebox{90}{\parbox{6.cm}{\centering\bigarrowleftright{Latent Dimension 2}}}}
    & \cellcolor[rgb]{0.993,0.906,0.144} \raisebox{0pt}[0.7cm][0.7cm]{\centering{$2.23 \times 10^{-1}$}} 
    & \cellcolor[rgb]{0.148,0.512,0.557} \raisebox{0pt}[0.7cm][0.7cm]{\centering\textcolor{white}{$1.37 \times 10^{-1}$}} 
    & \cellcolor[rgb]{0.207,0.372,0.553} \raisebox{0pt}[0.7cm][0.7cm]{\centering\textcolor{white}{$1.14 \times 10^{-1}$}} 
    & \cellcolor[rgb]{0.252,0.270,0.532} \raisebox{0pt}[0.7cm][0.7cm]{\centering\textcolor{white}{$1.00 \times 10^{-1}$}} 
    & \cellcolor[rgb]{0.267,0.005,0.329} \raisebox{0pt}[0.7cm][0.7cm]{\centering\textcolor{white}{$6.85 \times 10^{-2}$}} \\
    & \cellcolor[rgb]{0.158,0.684,0.502} \raisebox{0pt}[0.7cm][0.7cm]{\centering\textcolor{white}{$1.65 \times 10^{-1}$}} 
    & \cellcolor[rgb]{0.720,0.870,0.163} \raisebox{0pt}[0.7cm][0.7cm]{\centering\textcolor{white}{$2.06 \times 10^{-1}$}} 
    & \cellcolor[rgb]{0.168,0.460,0.558} \raisebox{0pt}[0.7cm][0.7cm]{\centering\textcolor{white}{$1.29 \times 10^{-1}$}} 
    & \cellcolor[rgb]{0.226,0.331,0.547} \raisebox{0pt}[0.7cm][0.7cm]{\centering\textcolor{white}{$1.08 \times 10^{-1}$}} 
    & \cellcolor[rgb]{0.256,0.261,0.528} \raisebox{0pt}[0.7cm][0.7cm]{\centering\textcolor{white}{$9.86 \times 10^{-2}$}} \\
    & \cellcolor[rgb]{0.167,0.464,0.558} \raisebox{0pt}[0.7cm][0.7cm]{\centering\textcolor{white}{$1.29 \times 10^{-1}$}} 
    & \cellcolor[rgb]{0.142,0.526,0.556} \raisebox{0pt}[0.7cm][0.7cm]{\centering\textcolor{white}{$1.39 \times 10^{-1}$}} 
    & \cellcolor[rgb]{0.369,0.789,0.383} \raisebox{0pt}[0.7cm][0.7cm]{\centering\textcolor{white}{$1.84 \times 10^{-1}$}} 
    & \cellcolor[rgb]{0.184,0.422,0.557} \raisebox{0pt}[0.7cm][0.7cm]{\centering\textcolor{white}{$1.22 \times 10^{-1}$}} 
    & \cellcolor[rgb]{0.241,0.296,0.540} \raisebox{0pt}[0.7cm][0.7cm]{\centering\textcolor{white}{$1.04 \times 10^{-1}$}} \\
    & \cellcolor[rgb]{0.205,0.376,0.554} \raisebox{0pt}[0.7cm][0.7cm]{\centering\textcolor{white}{$1.15 \times 10^{-1}$}} 
    & \cellcolor[rgb]{0.184,0.422,0.557} \raisebox{0pt}[0.7cm][0.7cm]{\centering\textcolor{white}{$1.23 \times 10^{-1}$}} 
    & \cellcolor[rgb]{0.156,0.490,0.558} \raisebox{0pt}[0.7cm][0.7cm]{\centering\textcolor{white}{$1.33 \times 10^{-1}$}} 
    & \cellcolor[rgb]{0.123,0.585,0.547} \raisebox{0pt}[0.7cm][0.7cm]{\centering\textcolor{white}{$1.49 \times 10^{-1}$}} 
    & \cellcolor[rgb]{0.201,0.384,0.554} \raisebox{0pt}[0.7cm][0.7cm]{\centering\textcolor{white}{$1.17 \times 10^{-1}$}} \\
    & \cellcolor[rgb]{0.236,0.310,0.543} \raisebox{0pt}[0.7cm][0.7cm]{\centering\textcolor{white}{$1.05 \times 10^{-1}$}} 
    & \cellcolor[rgb]{0.218,0.347,0.550} \raisebox{0pt}[0.7cm][0.7cm]{\centering\textcolor{white}{$1.11 \times 10^{-1}$}} 
    & \cellcolor[rgb]{0.199,0.388,0.555} \raisebox{0pt}[0.7cm][0.7cm]{\centering\textcolor{white}{$1.17 \times 10^{-1}$}} 
    & \cellcolor[rgb]{0.173,0.449,0.558} \raisebox{0pt}[0.7cm][0.7cm]{\centering\textcolor{white}{$1.26 \times 10^{-1}$}} 
    & \cellcolor[rgb]{0.148,0.512,0.557} \raisebox{0pt}[0.7cm][0.7cm]{\centering\textcolor{white}{$1.37 \times 10^{-1}$}} \\
    \end{tabular}}
    \caption{\textbf{Moving Across MatVAE latent space.} We manually set a triplet of valid mechanical properties (for the object in the middle) which is encoded by MatVAE. We use the produced latent and move across the two-dimensional latent space to build a $5\times5$ grid of valid mechanical property triplets. We show the mean displacement from the simulation of bunnies with these mechanical property triplets falling to the ground. (\video{00:00})}
    \label{fig:grid_cubes_fall_setting1}
        \vspace{-1em}
\end{wrapfigure}

==> fig/iclr/matvae_interp.tex <==
% Figure for interp_cubes_fall pair 1 as wrapfigure
\begin{wrapfigure}{r}{0.5\textwidth}
    \centering
    \scriptsize
    \resizebox{0.5\textwidth}{!}{%
    \setlength{\tabcolsep}{0pt}
    \begin{tabular}{c|ccc|c}
        \multicolumn{5}{c}{\normalsize\textbf{MatVAE}} \\
        Aerographite &
        \makecell{Carbon Fiber \\ (High Strength)} &
        \makecell{Carbon Fiber \\ (High Modulus)} &
        Carbon Nitride &
        Diamond\\
        $E = 0.001$ GPa & $E = 235.0$ GPa & $E = 400.0$ GPa &
        $E = 822.0$ GPa & $E = 1220.0$ GPa\\
        $\nu = 0.25$ & $\nu = 0.25$ & $\nu = 0.25$ &
        $\nu = 0.28$ & $\nu = 0.20$\\
        $\rho = 0.2$ kg/m$^3$ & $\rho = 1775$ kg/m$^3$ &
        $\rho = 1800$ kg/m$^3$ & $\rho = 3200$ kg/m$^3$ &
        $\rho = 3500$ kg/m$^3$\\
        \midrule
        \multicolumn{5}{c}{\normalsize\textbf{Naive Interpolation}} \\
        Aerographite &
        {\color{red}Invalid (\xmark)} &
        {\color{red}Invalid (\xmark)} &
        {\color{red}Invalid (\xmark)} &
        Diamond\\
        $E = 0.001$ GPa & $E = 305.0$ GPa & $E = 610.0$ GPa &
        $E = 915.0$ GPa & $E = 1220.0$ GPa\\
        $\nu = 0.25$ & $\nu = 0.24$ & $\nu = 0.23$ &
        $\nu = 0.21$ & $\nu = 0.20$\\
        $\rho = 0.2$ kg/m$^3$ & $\rho = 875$ kg/m$^3$ &
        $\rho = 1750$ kg/m$^3$ & $\rho = 2625$ kg/m$^3$ &
        $\rho = 3500$ kg/m$^3$\\
    \end{tabular}%
    }
    \caption{\textbf{MatVAE Allows Interpolation.} We set the left-most and right-most mechanical property triplets and use MatVAE latent space to linearly interpolate between the materials. We use "Invalid" to indicate properties that do not fall into any ranges from our vast MTD (\Cref{sec:mtd}). (\video{00:00})}
    \label{fig:interp_pair1}
\end{wrapfigure}

==> fig/iclr/reps.tex <==
\begin{wrapfigure}[]{l}{0.5\textwidth}
    \centering
    \includegraphics[width=0.5\textwidth]{assets/reps.pdf}
    \captionof{figure}{\acronym\ can operate on any geometry as long as it can be voxelized and rendered. We show \acronym\ can work on meshes, SDF, NeRF~\cite{mildenhall2020nerf}, and Gaussian Splats~\cite{kerbl3Dgaussians}.}
    \label{fig:reps}
\end{wrapfigure}

==> fig/iclr/tb_validity.tex <==
\begin{table*}[tb]
\centering
\input{fig/iclr/validity_content}
\caption{\textbf{Comparison of Validity of Predictions.} We report mean values and relative errors (in \%) for Young's modulus, Poisson's ratio, and density for the difference to the closest material range.}
\label{tab:validity}
\end{table*}

==> fig/matvaeinterp.tex <==
\newcolumntype{P}{>{\centering\arraybackslash}m{1.5cm}}
\newcolumntype{C}{>{\centering\arraybackslash}m{\cellsize}}

% Figure for Setting 1
\begin{figure}[tb]
    \centering
    \setlength{\tabcolsep}{0pt}%
    \renewcommand{\arraystretch}{0}%
    \newlength{\arrowcol}
\setlength{\arrowcol}{0.08\columnwidth} % width of the arrow column
\newlength{\cellsize}
\setlength{\cellsize}{\dimexpr(\columnwidth-\arrowcol)/5\relax}
\newcommand{\squarecell}[2]{%
  \cellcolor{#1}{%
    \color{white}\parbox[c][\cellsize][c]{\cellsize}{\centering #2}%
  }%
}
\resizebox{\linewidth}{!}{%
\begin{tabular}{c c c c c c}
% Top header row
& \multicolumn{5}{c}{\bigarrowleftright{Latent Dimension 1}} \\
% Left multirow rotated label + data rows
\multirow{5}{*}{\rotatebox{90}{\parbox{6.cm}{\centering\bigarrowleftright{Latent Dimension 2}}}}
& \cellcolor[rgb]{0.993,0.906,0.144} \raisebox{0pt}[0.7cm][0.7cm]{\centering{$2.23 \times 10^{-1}$}} 
& \cellcolor[rgb]{0.148,0.512,0.557} \raisebox{0pt}[0.7cm][0.7cm]{\centering\textcolor{white}{$1.37 \times 10^{-1}$}} 
& \cellcolor[rgb]{0.207,0.372,0.553} \raisebox{0pt}[0.7cm][0.7cm]{\centering\textcolor{white}{$1.14 \times 10^{-1}$}} 
& \cellcolor[rgb]{0.252,0.270,0.532} \raisebox{0pt}[0.7cm][0.7cm]{\centering\textcolor{white}{$1.00 \times 10^{-1}$}} 
& \cellcolor[rgb]{0.267,0.005,0.329} \raisebox{0pt}[0.7cm][0.7cm]{\centering\textcolor{white}{$6.85 \times 10^{-2}$}} \\
& \cellcolor[rgb]{0.158,0.684,0.502} \raisebox{0pt}[0.7cm][0.7cm]{\centering\textcolor{white}{$1.65 \times 10^{-1}$}} 
& \cellcolor[rgb]{0.720,0.870,0.163} \raisebox{0pt}[0.7cm][0.7cm]{\centering\textcolor{white}{$2.06 \times 10^{-1}$}} 
& \cellcolor[rgb]{0.168,0.460,0.558} \raisebox{0pt}[0.7cm][0.7cm]{\centering\textcolor{white}{$1.29 \times 10^{-1}$}} 
& \cellcolor[rgb]{0.226,0.331,0.547} \raisebox{0pt}[0.7cm][0.7cm]{\centering\textcolor{white}{$1.08 \times 10^{-1}$}} 
& \cellcolor[rgb]{0.256,0.261,0.528} \raisebox{0pt}[0.7cm][0.7cm]{\centering\textcolor{white}{$9.86 \times 10^{-2}$}} \\
& \cellcolor[rgb]{0.167,0.464,0.558} \raisebox{0pt}[0.7cm][0.7cm]{\centering\textcolor{white}{$1.29 \times 10^{-1}$}} 
& \cellcolor[rgb]{0.142,0.526,0.556} \raisebox{0pt}[0.7cm][0.7cm]{\centering\textcolor{white}{$1.39 \times 10^{-1}$}} 
& \cellcolor[rgb]{0.369,0.789,0.383} \raisebox{0pt}[0.7cm][0.7cm]{\centering\textcolor{white}{$1.84 \times 10^{-1}$}} 
& \cellcolor[rgb]{0.184,0.422,0.557} \raisebox{0pt}[0.7cm][0.7cm]{\centering\textcolor{white}{$1.22 \times 10^{-1}$}} 
& \cellcolor[rgb]{0.241,0.296,0.540} \raisebox{0pt}[0.7cm][0.7cm]{\centering\textcolor{white}{$1.04 \times 10^{-1}$}} \\
& \cellcolor[rgb]{0.205,0.376,0.554} \raisebox{0pt}[0.7cm][0.7cm]{\centering\textcolor{white}{$1.15 \times 10^{-1}$}} 
& \cellcolor[rgb]{0.184,0.422,0.557} \raisebox{0pt}[0.7cm][0.7cm]{\centering\textcolor{white}{$1.23 \times 10^{-1}$}} 
& \cellcolor[rgb]{0.156,0.490,0.558} \raisebox{0pt}[0.7cm][0.7cm]{\centering\textcolor{white}{$1.33 \times 10^{-1}$}} 
& \cellcolor[rgb]{0.123,0.585,0.547} \raisebox{0pt}[0.7cm][0.7cm]{\centering\textcolor{white}{$1.49 \times 10^{-1}$}} 
& \cellcolor[rgb]{0.201,0.384,0.554} \raisebox{0pt}[0.7cm][0.7cm]{\centering\textcolor{white}{$1.17 \times 10^{-1}$}} \\
& \cellcolor[rgb]{0.236,0.310,0.543} \raisebox{0pt}[0.7cm][0.7cm]{\centering\textcolor{white}{$1.05 \times 10^{-1}$}} 
& \cellcolor[rgb]{0.218,0.347,0.550} \raisebox{0pt}[0.7cm][0.7cm]{\centering\textcolor{white}{$1.11 \times 10^{-1}$}} 
& \cellcolor[rgb]{0.199,0.388,0.555} \raisebox{0pt}[0.7cm][0.7cm]{\centering\textcolor{white}{$1.17 \times 10^{-1}$}} 
& \cellcolor[rgb]{0.173,0.449,0.558} \raisebox{0pt}[0.7cm][0.7cm]{\centering\textcolor{white}{$1.26 \times 10^{-1}$}} 
& \cellcolor[rgb]{0.148,0.512,0.557} \raisebox{0pt}[0.7cm][0.7cm]{\centering\textcolor{white}{$1.37 \times 10^{-1}$}} \\
\end{tabular}}
    \caption{\textbf{Moving Across MatVAE latent space.} We manually set a triplet of valid mechanical properties (for the object in the middle) which is encoded by MatVAE. We use the produced latent and move across the two-dimensional latent space to build a $5\times5$ grid of valid mechanical property triplets. We show the mean displacement from the simulation of bunnies with these mechanical property triplets falling to the ground. (\video{00:00})}
    \label{fig:grid_cubes_fall_setting1}
\end{figure}


% figure for interp_cubes_fall pair 1
\begin{figure}[tb]
    \centering
    \scriptsize
    \resizebox{\columnwidth}{!}{%
    \setlength{\tabcolsep}{0pt}
    \begin{tabular}{c|ccc|c}
        \multicolumn{5}{c}{\normalsize\textbf{MatVAE}} \\
        Aerographite &
        \makecell{Carbon Fiber \\ (High Strength)} &
        \makecell{Carbon Fiber \\ (High Modulus)} &
        Carbon Nitride &
        Diamond\\
        $E = 0.001$ GPa & $E = 235.0$ GPa & $E = 400.0$ GPa &
        $E = 822.0$ GPa & $E = 1220.0$ GPa\\
        $\nu = 0.25$ & $\nu = 0.25$ & $\nu = 0.25$ &
        $\nu = 0.28$ & $\nu = 0.20$\\
        $\rho = 0.2$ kg/m$^3$ & $\rho = 1775$ kg/m$^3$ &
        $\rho = 1800$ kg/m$^3$ & $\rho = 3200$ kg/m$^3$ &
        $\rho = 3500$ kg/m$^3$\\
        \midrule
        \multicolumn{5}{c}{\normalsize\textbf{Naive Interpolation}} \\
        Aerographite &
        {\color{red}Invalid (\xmark)} &
        {\color{red}Invalid (\xmark)} &
        {\color{red}Invalid (\xmark)} &
        Diamond\\
        $E = 0.001$ GPa & $E = 305.0$ GPa & $E = 610.0$ GPa &
        $E = 915.0$ GPa & $E = 1220.0$ GPa\\
        $\nu = 0.25$ & $\nu = 0.24$ & $\nu = 0.23$ &
        $\nu = 0.21$ & $\nu = 0.20$\\
        $\rho = 0.2$ kg/m$^3$ & $\rho = 875$ kg/m$^3$ &
        $\rho = 1750$ kg/m$^3$ & $\rho = 2625$ kg/m$^3$ &
        $\rho = 3500$ kg/m$^3$\\
    \end{tabular}%
    }
    \caption{\textbf{MatVAE Allows Interpolation.} We set the left-most and right-most mechanical property triplets and use MatVAE latent space to linearly interpolate between the materials. We use "Invalid" to indicate properties that do not fall into any ranges from our vast MTD (\Cref{sec:mtd}). (\video{00:00})}
    \label{fig:interp_pair1}
\end{figure}

==> fig/matvaelatentspace.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{assets/latent_space_by_materials.pdf}
    \caption{\textbf{Generating from MatVAE latent space.} We demonstrate decoding or generating from MatVAE at any point in the latent space leads to a plausible material triplet that fits in the ranges for some physical material.}
    \label{fig:genfrommatvae}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{assets/real_materials_latent_space.pdf}
    \caption{\textbf{Encoding materials to MatVAE latent space.} We choose some real world materials and demonstrate encoding triplets sampled from their ranges to the latent space. We observe some overlap since mechanical properties for two different materials may overlap.}
    \label{fig:encodematvae}
\end{figure}

==> fig/plinko.tex <==
\begin{figure}[tb]
    \centering
    \includegraphics{assets/plinko.pdf}
    \bigarrow{time}
    \caption{\textbf{Simulating a Plinko.} We simulate 18 3D Gaussian Splats with properties estimated by \acronym\ falling through a plinko machine.  (\video{00:00})}
    \label{fig:plinko}
\end{figure}

==> fig/reps.tex <==
\begin{figure}
    \centering
    \includegraphics{assets/reps.pdf}
    \caption{\acronym\ can operate on any geometry as long as it can be voxelized and rendered. We show \acronym\ can work on meshes, SDF, NeRF~\cite{mildenhall2020nerf}, and Gaussian Splats~\cite{kerbl3Dgaussians}.}
    \label{fig:reps}
\end{figure}

==> fig/simulators.tex <==
\begin{figure}[tb]
    \centering
    \includegraphics{assets/simulators.pdf}
    \caption{\textbf{Simulator Differences.} We simulate a solid sphere with XPBD~\cite{xpbd}, MPM~\cite{mpm}, and FEM setting the material properties to $E=10^4$ Pa, $\nu=0.3$, and $\rho=10^3 \operatorname{kg/m}^3$ (\video{00:00}).}
    % \todo{Rishit: add space between columns for a smaller figure (due to aspect ratio).}
    \vspace{-1.5em}
    \label{fig:simulators}
\end{figure}

==> shortcuts.tex <==
% shortcuts for bold characters (vectors, matrices)


% Our selection
\newcommand{\selthree}{S^{\,\mbox{\footnotesize \mancube}}}
\newcommand{\seltwo}{S^{\scriptsize \boxplus}}
\newcommand{\seltwoauto}{S^{\scriptsize \boxdot}}

% shortcuts for bold greek characters (vectors, matrices)
\newcommand{\balpha}{\boldsymbol{\alpha}}\newcommand{\bAlpha}{\boldsymbol{\Alpha}}
\newcommand{\bbeta}{\boldsymbol{\beta}}\newcommand{\bBeta}{\boldsymbol{\Beta}}
\newcommand{\bgamma}{\boldsymbol{\gamma}}\newcommand{\bGamma}{\boldsymbol{\Gamma}}
\newcommand{\bdelta}{\boldsymbol{\delta}}\newcommand{\bDelta}{\boldsymbol{\Delta}}
\newcommand{\bepsilon}{\boldsymbol{\epsilon}}\newcommand{\bEpsilon}{\boldsymbol{\Epsilon}}
\newcommand{\bzeta}{\boldsymbol{\zeta}}\newcommand{\bZeta}{\boldsymbol{\Zeta}}
\newcommand{\beeta}{\boldsymbol{\eta}}\newcommand{\bEta}{\boldsymbol{\Eta}} % \beta already taken
\newcommand{\btheta}{\boldsymbol{\theta}}\newcommand{\bTheta}{\boldsymbol{\Theta}}
\newcommand{\biota}{\boldsymbol{\iota}}\newcommand{\bIota}{\boldsymbol{\Iota}}
\newcommand{\bkappa}{\boldsymbol{\kappa}}\newcommand{\bKappa}{\boldsymbol{\Kappa}}
\newcommand{\blambda}{\boldsymbol{\lambda}}\newcommand{\bLambda}{\boldsymbol{\Lambda}}
\newcommand{\bmu}{\boldsymbol{\mu}}\newcommand{\bMu}{\boldsymbol{\Mu}}
\newcommand{\bnu}{\boldsymbol{\nu}}\newcommand{\bNu}{\boldsymbol{\Nu}}
\newcommand{\bxi}{\boldsymbol{\xi}}\newcommand{\bXi}{\boldsymbol{\Xi}}
\newcommand{\bomikron}{\boldsymbol{\omikron}}\newcommand{\bOmikron}{\boldsymbol{\Omikron}}
\newcommand{\bpi}{\boldsymbol{\pi}}\newcommand{\bPi}{\boldsymbol{\Pi}}
\newcommand{\brho}{\boldsymbol{\rho}}\newcommand{\bRho}{\boldsymbol{\Rho}}
\newcommand{\bsigma}{\boldsymbol{\sigma}}\newcommand{\bSigma}{\boldsymbol{\Sigma}}
\newcommand{\btau}{\boldsymbol{\tau}}\newcommand{\bTau}{\boldsymbol{\Tau}}
\newcommand{\bypsilon}{\boldsymbol{\ypsilon}}\newcommand{\bYpsilon}{\boldsymbol{\Ypsilon}}
\newcommand{\bphi}{\boldsymbol{\phi}}\newcommand{\bPhi}{\boldsymbol{\Phi}}
\newcommand{\bchi}{\boldsymbol{\chi}}\newcommand{\bChi}{\boldsymbol{\Chi}}
\newcommand{\bpsi}{\boldsymbol{\psi}}\newcommand{\bPsi}{\boldsymbol{\Psi}}
\newcommand{\bomega}{\boldsymbol{\omega}}\newcommand{\bOmega}{\boldsymbol{\Omega}}

% shortcuts for blackboard bold characters (eg, number sets)
\newcommand{\nA}{\mathbb{A}}
\newcommand{\nB}{\mathbb{B}}
\newcommand{\nC}{\mathbb{C}}
\newcommand{\nD}{\mathbb{D}}
\newcommand{\nE}{\mathbb{E}}
\newcommand{\nF}{\mathbb{F}}
\newcommand{\nG}{\mathbb{G}}
\newcommand{\nH}{\mathbb{H}}
\newcommand{\nI}{\mathbb{I}}
\newcommand{\nJ}{\mathbb{J}}
\newcommand{\nK}{\mathbb{K}}
\newcommand{\nL}{\mathbb{L}}
\newcommand{\nM}{\mathbb{M}}
\newcommand{\nN}{\mathbb{N}}
\newcommand{\nO}{\mathbb{O}}
\newcommand{\nP}{\mathbb{P}}
\newcommand{\nQ}{\mathbb{Q}}
\newcommand{\nR}{\mathbb{R}}
\newcommand{\nS}{\mathbb{S}}
\newcommand{\nT}{\mathbb{T}}
\newcommand{\nU}{\mathbb{U}}
\newcommand{\nV}{\mathbb{V}}
\newcommand{\nW}{\mathbb{W}}
\newcommand{\nX}{\mathbb{X}}
\newcommand{\nY}{\mathbb{Y}}
\newcommand{\nZ}{\mathbb{Z}}

% shortcuts for calligraphic characters (sets, index sets, ...)
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\co}{\mathcal{o}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cZ}{\mathcal{Z}}

% references to figures, sections, algorithms, equations, tables
% \newcommand{\figref}[1]{Fig.~\ref{#1}}
% \newcommand{\secref}[1]{Section~\ref{#1}}
% \newcommand{\algref}[1]{Algorithm~\ref{#1}}
% \newcommand{\eqnref}[1]{Eq.~\eqref{#1}}
% \newcommand{\tabref}[1]{Table~\ref{#1}}

% argmin / argmax operators
\usepackage{amsfonts}
\DeclareMathOperator*{\argmax}{argmax~}
\DeclareMathOperator*{\argmin}{argmin~}
\DeclareMathOperator{\EX}{\mathbb{E}}
\DeclareMathOperator{\Tr}{Tr}
\DeclareMathOperator{\relu}{relu}

% mathcal / mathbf shortcuts
\def\mc{\mathcal}
\def\mb{\mathbf}

% nice transpose operator
\newcommand{\T}{^{\raisemath{-1pt}{\mathsf{T}}}}

% statistical dependency symbol (_||_)
%\newcommand{\Perp}{\perp\!\!\! \perp}

% shortcuts for: \eg, \ie, \cf, \etc, \vs, \wrt, \dof, \etal, \iid
\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}
\def\eg{e.g\onedot} \def\Eg{E.g\onedot}
\def\ie{i.e\onedot} \def\Ie{I.e\onedot}
\def\cf{cf\onedot} \def\Cf{Cf\onedot}
\def\etc{etc\onedot}
\def\vs{vs\onedot}
\def\wrt{wrt\onedot}
\def\dof{d.o.f\onedot}
\def\etal{et~al\onedot}
\def\iid{i.i.d\onedot}
\makeatother

% nice url font and color
\renewcommand\UrlFont{\color{blue}\rmfamily}

% rotation
\newcommand*\rot{\rotatebox{90}}

% boldparagraph for unnumbered sections
\newcommand{\boldparagraph}[1]{\vspace{0.2cm}\noindent{\bf #1:} }

\newcommand{\figref}[1]{Fig.~\ref{#1}}
\newcommand{\tabref}[1]{Tab.~\ref{#1}}
\newcommand{\secref}[1]{Sec.~\ref{#1}}

% custom color definitions
\usepackage{xcolor}
\definecolor{darkred}{rgb}{0.7,0.2,0.1}
\definecolor{darkgreen}{rgb}{0,0.7,0}
\definecolor{orange}{RGB}{255,127,0}
\definecolor{ourpurple}{RGB}{127,127,204}
\definecolor{ourteal}{RGB}{60,160,160}
\definecolor{palgreen}{RGB}{51,179,179}
\definecolor{magenta}{RGB}{199,21,133}

% commands for comments
% \newcommand{\todo}[1]{{\color{red}{#1}}}
\newcommand{\finalize}[1]{{\color{orange}{#1}}}
\newcommand{\masha}[1]{{\color{blue} {\bf Masha:} {#1}} }
\newcommand{\dave}[1]{{\color{orange} {\bf Dave:} {#1}} }
\newcommand{\nish}[1]{{\color{ourteal} {\bf Nishkrit:} {#1}} }
\newcommand{\seung}[1]{{\color{green} {\bf Seung:} {#1}} }
\newcommand{\orp}[1]{{\color{purple}{#1}} }
\newcommand{\orpc}[1]{{\color{purple} {\bf Or:} {#1}} }
%\newcommand{\maybeincl}[1]{#1}



\newcommand{\conf}[1]{{\color{blue}{#1}}}
\newcommand{\edit}[1]{{\color{blue}{#1}}}
%\renewcommand{\edit}[1]{{#1}}

\newcommand{\bluelink}[1]{{\color{blue}{#1}}}

\newcommand{\ourmodel}{ArtisanGS}
\newcommand{\ourm}{ArtisanGS}
% Artisan

\def\checkmark{\tikz\fill[scale=0.4](0,.35) -- (.25,0) -- (1,.7) -- (.25,.15) -- cycle;}

\newcommand{\yes}{\checkmark}%
\newcommand{\no}{\color{red}$\times$}%

%\renewcommand{\algorithmiccomment}[1]{\hfill$\triangleright$\textit{#1}}
\renewcommand{\algorithmiccomment}[1]{\hfill{\color{ourteal}{$\triangleright$ #1}}}
\newcommand{\Commentcustom}[1]{{\color{ourteal}{$\triangleright$ #1}}}

==> tab/iclr/mass.tex <==
\begin{table}[tb]
\vspace{-1em}
\centering
\input{tab/iclr/mass_content}
\caption{\textbf{Mass Estimation.} We show the errors for estimating mass of objects on the ABO-500~\cite{Collins_2022_CVPR} dataset.}
\label{tab:mass}
\vspace{-1em}
\end{table}

==> tab/iclr/matvaeablations.tex <==
\newcommand{\matvaedistrowablation}{
\textbf{0.0405} & \textbf{0.0798} & \underline{0.1379} & 
\textbf{0.0317} & \textbf{0.0437} & \textbf{0.0342} & 
\textbf{0.0132} & \textbf{0.0172} & \underline{0.0260}
}
\newcommand{\matvaemetricsrowablation}{
\textbf{0.0034} & \textbf{0.0426} & \textbf{0.0330} & 
\textbf{0.0054} & \textbf{0.0036} & \textbf{0.0036} & 
\textbf{0.0131} & \textbf{0.4439} & \textbf{0.0411}
}
\newcommand{\vanillavaedistrow}{
\underline{0.0653} & \underline{0.0868} & \textbf{0.0547} & 
\underline{0.0849} & \underline{0.1057} & \underline{0.0689} & 
\underline{0.0547} & \underline{0.0744} & \textbf{0.0175}
}
\newcommand{\vanillavaemetricsrow}{
\underline{0.0512} & \underline{15366.8750} & \underline{0.8306} & 
\underline{0.0542} & \underline{0.0544} & \underline{0.0447} & 
\underline{0.2384} & \underline{2.1893} & \underline{0.4690}
}
\newcommand{\matvaedistbenefitrow}{
{\textbf{\textcolor{green}{(-0.025)}}} & 
{\textbf{\textcolor{green}{(-0.007)}}} & 
{\textbf{\textcolor{red}{(+0.083)}}} & 
{\textbf{\textcolor{green}{(-0.053)}}} & 
{\textbf{\textcolor{green}{(-0.062)}}} & 
{\textbf{\textcolor{green}{(-0.035)}}} & 
{\textbf{\textcolor{green}{(-0.042)}}} & 
{\textbf{\textcolor{green}{(-0.057)}}} & 
{\textbf{\textcolor{red}{(+0.009)}}}
}
\newcommand{\matvaemetricsbenefitrow}{
{\textbf{\textcolor{green}{(-0.048)}}} & 
{\textbf{\textcolor{green}{(-15366.8)}}} & 
{\textbf{\textcolor{green}{(-0.798)}}} & 
{\textbf{\textcolor{green}{(-0.049)}}} & 
{\textbf{\textcolor{green}{(-0.051)}}} & 
{\textbf{\textcolor{green}{(-0.041)}}} & 
{\textbf{\textcolor{green}{(-0.225)}}} & 
{\textbf{\textcolor{green}{(-1.745)}}} & 
{\textbf{\textcolor{green}{(-0.428)}}}
}
\begin{table*}[tb]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{lrrrrrrrrr}
\toprule
\rowcolor{blue!15}
Model & 
\multicolumn{3}{c}{Young's Modulus ($E$)} & 
\multicolumn{3}{c}{Poisson's Ratio ($\nu$)} & 
\multicolumn{3}{c}{Density ($\rho$)}\\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10}
\rowcolor{blue!15}
& W$_1$ ($\downarrow$) & W$_2$ ($\downarrow$) & $D_{\text{KL}}$ ($\downarrow$) 
& W$_1$ ($\downarrow$) & W$_2$ ($\downarrow$) & $D_{\text{KL}}$ ($\downarrow$) 
& W$_1$ ($\downarrow$) & W$_2$ ($\downarrow$) & $D_{\text{KL}}$ ($\downarrow$) \\
\midrule
Vanilla VAE~\cite{kingma2022autoencodingvariationalbayes} & \vanillavaedistrow \\
MatVAE & \matvaedistrowablation \\
& \matvaedistbenefitrow \\
w/o NF & 0.0339 & 0.0447 & 0.0441 & 0.0417 & 0.0504 & 0.0848 & 0.0599 & 0.0819 & 0.0529\\
w/o TC penalty & 0.0633 & 0.0855 & 0.0500 & 0.0844 & 0.1052 & 0.0672 & 0.0525 & 0.0715 & 0.0109 \\
w/o free nats & 0.0749 & 0.1168 & 0.1311 & 0.2014 & 0.2064 & 0.6376 & 0.0421 & 0.0507 & 0.0223 \\\midrule
\rowcolor{blue!15} 
& $\log(E)$ ($\downarrow$) & $\nu$ ($\downarrow$) & $\rho$ ($\downarrow$) 
& $\log(E/\rho)$ ($\downarrow$) & $\log(G)$ ($\downarrow$) & $\log(K)$ ($\downarrow$) 
& L.S. ($\downarrow$) & E.A. ($\downarrow$) & Bray–Curtis ($\downarrow$) \\
\midrule
Vanilla VAE~\cite{kingma2022autoencodingvariationalbayes} & \vanillavaemetricsrow \\
MatVAE & \matvaemetricsrowablation \\
& \matvaemetricsbenefitrow \\
w/o NF & 0.0020 & \texttt{nan} & 0.0160 & 0.0033 & 0.0021 & 0.0021 & 0.0086 & 0.1729 & 0.0234\\
w/o TC penalty & 0.0499 & 15567.0986 & 0.8298 & 0.0537 & 0.0530 & 0.0437 & 0.2382 & 2.1514 & 0.4562\\
w/o free nats & 0.0036 & 16332.7829 & 0.0276 & 0.0053 & 0.0037 & 0.0041 & 0.0116 & 0.2966 & 0.0436\\
\bottomrule
\end{tabular}
}
\caption{\textbf{MatVAE Ablation.} We ablate MatVAE by comparing it against a vanilla VAE and present reconstruction and distirbutional metrics.}
\label{tab:matvaeablation}
\end{table*}

==> tab/iclr/matvaemetrics.tex <==
\newcommand{\matvaedistrow}{
0.0405 & 0.0798 & 0.1379 & 
0.0317 & 0.0437 & 0.0342 & 
0.0132 & 0.0172 & 0.0260
}
\newcommand{\matvaemetricsrow}{
0.0034 & 0.0426 & 0.0330 & 
0.0054 & 0.0036 & 0.0036 & 
0.0131 & 0.4439 & 0.0411
}

\begin{table*}[hb!]
\centering
\input{tab/iclr/matvaemetrics_content}
\caption{\textbf{MatVAE reconstruction errors} on the MTD test set show excellent accuracy across all metrics (\Cref{app:metricsmech}).}
\label{tab:matvaemetrics}
\end{table*}

==> tab/iclr/propertyestimation.tex <==
\input{tab/iclr/propertyestimation_voxel}
\input{tab/iclr/propertyestimation_object}



==> tab/iclr/propertyestimation_object.tex <==

\begin{table*}[tb]
\centering
\input{tab/iclr/propertyestimation_object_content}
\end{table*}

==> tab/mass.tex <==
\begin{table}[tb]
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{lrrrr}
\toprule
\rowcolor{blue!15}Method & ALDE ($\downarrow$) & ADE ($\downarrow$) & ARE ($\downarrow$) & MnRE \textbf{($\uparrow$)}\\
\midrule
NeRF2Physics~\cite{zhai2024physicalpropertyunderstandinglanguageembedded} & 0.736 & 12.725 & 1.040 & 0.564\\
PUGS~\cite{shuai2025pugszeroshotphysicalunderstanding} & \underline{0.661} & \underline{9.461} & \textbf{0.767} & \textbf{0.576}\\
\midrule Ours & \textbf{0.631} & \textbf{8.433} & \underline{0.887} & \textbf{0.576}\\
\bottomrule
\end{tabular}}
\caption{\textbf{Mass Estimation.} We show the errors for estimating mass of objects on the ABO-500~\cite{Collins_2022_CVPR} dataset.}
\label{tab:mass}
\end{table}

==> tab/matvaemetrics.tex <==
\newcommand{\matvaedistrow}{
0.0405 & 0.0798 & 0.1379 & 
0.0317 & 0.0437 & 0.0342 & 
0.0132 & 0.0172 & 0.0260
}
\newcommand{\matvaemetricsrow}{
0.0034 & 0.0426 & 0.0330 & 
0.0054 & 0.0036 & 0.0036 & 
0.0131 & 0.4439 & 0.0411
}

\begin{table*}[tb]
\centering
\begin{tabular}{rrrrrrrrr}
\toprule
\rowcolor{blue!15}
\multicolumn{3}{c}{Young's Modulus ($E$)}
& \multicolumn{3}{c}{Poisson's Ratio ($\nu$)}
& \multicolumn{3}{c}{Density ($\rho$)}\\ 
\cmidrule(lr){1-3}\cmidrule(lr){4-6}\cmidrule(lr){7-9}
\rowcolor{blue!15}W$_1$ ($\downarrow$) & W$_2$ ($\downarrow$) & $D_{\text{KL}}$ ($\downarrow$) & W$_1$ ($\downarrow$) & W$_2$ ($\downarrow$) & $D_{\text{KL}}$ ($\downarrow$) & W$_1$ ($\downarrow$) & W$_2$ ($\downarrow$) & $D_{\text{KL}}$ ($\downarrow$) \\
\midrule
\matvaedistrow\\
\bottomrule
\end{tabular}
\caption{\textbf{Distribution learned by MatVAE.} We compare distributions of the generated material triplets and the test set.}
\label{tab:matvaedistmetrics}
\end{table*}

\begin{table*}[tb]
\centering
\begin{tabular}{rrrrrrrrrr}
\toprule
\rowcolor{blue!15}$\log(E)$ ($\downarrow$) & $\nu$ ($\downarrow$) & $\rho$ ($\downarrow$) & $\log(E/\rho)$ ($\downarrow$) & $\log(G)$ ($\downarrow$) & $\log(K)$ ($\downarrow$) & L.S. ($\downarrow$) & E.A. ($\downarrow$) & Bray–Curtis ($\downarrow$) \\
\midrule
\matvaemetricsrow\\
\bottomrule
\end{tabular}
\caption{\textbf{Reconstructing Triplets.} We show errors for reconstructing material triplets from the test set. We explain the metrics in~\Cref{app:metricsmech}.}
\label{tab:matvaemetrics}
\end{table*}

==> tab/propertyestimation.tex <==
\newcommand{\voxelproprow}{
\textbf{0.3765} {\textbf{\scriptsize\textcolor{gray}{($\pm$0.39)}}} & 
\textbf{0.0421} {\textbf{\scriptsize\textcolor{gray}{($\pm$0.05)}}} & 
\textbf{0.0250} {\textbf{\scriptsize\textcolor{gray}{($\pm$0.01)}}} & 
\textbf{0.0837} {\textbf{\scriptsize\textcolor{gray}{($\pm$0.03)}}} & 
\textbf{113.3807} {\textbf{\scriptsize\textcolor{gray}{($\pm$301.90)}}} & 
\textbf{0.0908} {\textbf{\scriptsize\textcolor{gray}{($\pm$0.14)}}}
}
\begin{table*}[tb]
\centering
\begin{tabular}{lrrrrrr}
\toprule
\rowcolor{blue!15}Method & \multicolumn{2}{c}{Young's Modulus Pa ($E$)} & \multicolumn{2}{c}{Poisson's Ratio ($\nu$)} & \multicolumn{2}{c}{Density $\frac{kg}{m^3}$ ($\rho$)} \\
\cmidrule(r){2-3} \cmidrule(r){4-5} \cmidrule(r){6-7}
\rowcolor{blue!15}& ALDE ($\downarrow$) & ALRE ($\downarrow$) & ADE ($\downarrow$) & ARE ($\downarrow$) & ADE ($\downarrow$) & ARE ($\downarrow$) \\
\midrule
NeRF2Physics~\cite{zhai2024physicalpropertyunderstandinglanguageembedded} & \underline{2.5719} {\scriptsize{($\pm$1.15)}} & \underline{0.4122} {\scriptsize{($\pm$0.08)}} & - & - & 1354.9458 {\scriptsize{($\pm$1315.71)}} & 1.1496 {\scriptsize{($\pm$0.67)}} \\
PUGS~\cite{shuai2025pugszeroshotphysicalunderstanding} & 3.8619 {\scriptsize{($\pm$2.01)}} & 0.4512 {\scriptsize{($\pm$0.11)}} & - & - & 3641.0715 {\scriptsize{($\pm$3320.78)}} & 4.0413 {\scriptsize{($\pm$4.16)}} \\
Phys4DGen$^\star$~\cite{lin2025phys4dgenphysicscompliant4dgeneration} & 5.2977 {\scriptsize{($\pm$3.36)}} & 0.4825 {\scriptsize{($\pm$0.14)}} & \underline{0.0394} {\scriptsize{($\pm$0.05)}} & \underline{0.1425} {\scriptsize{($\pm$0.21)}} & \underline{1285.9489} {\scriptsize{($\pm$1981.11)}} & \underline{1.0445} {\scriptsize{($\pm$2.53)}} \\
\midrule
Ours &  \voxelproprow\\
\bottomrule
\end{tabular}
\caption{\textbf{Voxel Mechanical Property Estimation.} Errors for predicting mechanical properties from 3D objects averaged across all voxels in the test set.}
\label{tab:material-properties}
\end{table*}

\begin{table*}[tb]
\centering
\begin{tabular}{lrrrrrr}
\toprule
\rowcolor{blue!15}Method & \multicolumn{2}{c}{Young's Modulus Pa ($E$)} & \multicolumn{2}{c}{Poisson's Ratio ($\nu$)} & \multicolumn{2}{c}{Density $\frac{kg}{m^3}$ ($\rho$)} \\
\cmidrule(r){2-3} \cmidrule(r){4-5} \cmidrule(r){6-7}
\rowcolor{blue!15}& ALDE ($\downarrow$) & ALRE ($\downarrow$) & ADE ($\downarrow$) & ARE ($\downarrow$) & ADE ($\downarrow$) & ARE ($\downarrow$) \\
\midrule
NeRF2Physics~\cite{zhai2024physicalpropertyunderstandinglanguageembedded} & \underline{2.8000} {\scriptsize{($\pm$1.05)}} & \underline{0.1346} {\scriptsize{($\pm$0.05)}} & - & - & \underline{1432.0343} {\scriptsize{($\pm$964.88)}} & \underline{1.0365} {\scriptsize{($\pm$0.63)}} \\
PUGS~\cite{shuai2025pugszeroshotphysicalunderstanding} & 3.3942 {\scriptsize{($\pm$1.72)}} & 0.1688 {\scriptsize{($\pm$0.10)}} & - & - & 3568.2150 {\scriptsize{($\pm$2839.13)}} & 3.2429 {\scriptsize{($\pm$3.56)}} \\
Phys4DGen$^\star$~\cite{lin2025phys4dgenphysicscompliant4dgeneration} & 4.8967 {\scriptsize{($\pm$3.17)}} & 0.2227 {\scriptsize{($\pm$0.14)}} & \underline{0.0407} {\scriptsize{($\pm$0.04)}} & \underline{0.1467} {\scriptsize{($\pm$0.18)}} & 1865.5673 {\scriptsize{($\pm$2176.90)}} & 1.4394 {\scriptsize{($\pm$2.35)}} \\
\midrule
Ours & 
\textbf{0.3793} {\textbf{\scriptsize\textcolor{gray}{($\pm$0.29)}}} & 
\textbf{0.0409} {\textbf{\scriptsize\textcolor{gray}{($\pm$0.04)}}} & 
\textbf{0.0241} {\textbf{\scriptsize\textcolor{gray}{($\pm$0.01)}}} & 
\textbf{0.0818} {\textbf{\scriptsize\textcolor{gray}{($\pm$0.03)}}} & 
\textbf{142.6949} {\textbf{\scriptsize\textcolor{gray}{($\pm$166.90)}}} & 
\textbf{0.0921} {\textbf{\scriptsize\textcolor{gray}{($\pm$0.07)}}} \\
\bottomrule
\end{tabular}
\caption{\textbf{Object Mechanical Property Estimation.} Errors for predicting mechanical properties from 3D objects averaged across all voxels and all objects in the test set.}
\label{tab:material-properties-object}
\end{table*}


==> text/conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

We take a step toward unifying geometric representation and physical realism in digital assets by introducing the first framework to automatically endow arbitrary 3D objects with physically valid, volumetric material properties. By making simulation-based reasoning possible directly from standard 3D representations, our approach lowers the barrier for integrating accurate physics into digital workflows, with potential impact across digital twins, robotics, and beyond. As methods for material inference and representation continue to mature, we expect the boundary between visual and physical realism in virtual environments to become increasingly permeable, supporting more robust, generalizable, and accessible simulation-based reasoning. We hope this direction opens new avenues for interactive, physics-aware design and analysis.

==> text/discussion.tex <==
\section{Limitations and Future Work}
\label{sec:discussion}
% We introduce a representation-agnostic system that maps any 3D asset (mesh, SDF, Gaussian splat, or voxel grid) to a volumetric field of physically valid material triplets $(E,\nu,\rho)$. We achieve this by first voxelizing the input geometry and deriving per-voxel features by aggregating multi-view image features from a pretrained vision model. A Geometry Transformer then maps these rich visual features to a learned 2D latent space. From this space, a decoder, pre-trained as part of our MatVAE, generates the final material properties. Through extensive evaluation, we demonstrated that our framework produces accurate mechanical property estimations while requiring zero manual authoring to turn 3D assets into simulation-ready objects. We bridge the long-standing gap between geometry-centric asset libraries and physics-centric simulation engines, making assets truly "drag-and-drop sim-ready." The ability to generate physically plausible material fields without manual intervention opens the door to scalable automated simulation pipelines. \dave{ the discussion reads very similary to the conclusion or an abstract, I think we can safely remove it}

The most significant limitation of our approach is that it voxelizes input geometry at a fixed resolution. During annotation, this also requires us to assume individual common materials like wood are istropic. This can lead to oversmoothing of fine-scale material variations, particularly in thin shells or highly heterogeneous regions, and may result in underestimation of local stiffness or loss of critical structural detail.  Particularly, the property fields we estimate are not continuous. \emph{Second}, our method could be extended to learn a septet $(E, \nu, \rho, \sigma_y, G, \alpha_T, c_p)$, incorporating yield strength, shear modulus, thermal expansion, and specific heat. Currently, we predict true material properties; thus, using them requires an accurate simulator run to convergence. However, our method could be modified to learn hierarchical MatVAE's that learn simulator-specific properties (like SPH~\cite{monaghan1992smoothed} or MPM~\cite{sulsky1994particle} properties).

\emph{Third}, our model is constrained by its reliance on static visual datasets, which does not contain many instances of rare materials, and it currently lacks a mechanism to synthetically generate physically-grounded training data for these under-represented cases through differentiable simulation. Furthermore, we are unable to leverage richer supervisory signals from other modalities like tactile or acoustic data or a way to learn.
\emph{Finally}, our learned material manifold can directly be applied to inverse design problems like jointly optimizing geometry and material to meet target physical behaviours. The trained latent space can also directly be used to generate many similar kinds of plausible properties for problems in digital twin creation, robot learning, and automated content generation.

==> text/outline.tex <==
\noindent{\Large Outline}

\section{Introduction}

\masha{Really well summarized and the outline looks good. Please keep this as a reference and write a full intro.}

\begin{itemize}
\item \textbf{Context \& Motivation}
  \begin{itemize}
  \item Modern simulation pipelines and digital-twin workflows rely on \emph{physically-accurate material properties} (e.g., Young's modulus $E$, Poisson's ratio $\nu$, density $\rho$) to predict deformation, structural failure, acoustic response, and haptic feedback.
  \item Vast public 3D repositories (ShapeNet, Thingi10K, Objaverse, etc.) contain \emph{geometry} but almost never volumetric material metadata, forcing artists and engineers to guess or copy-paste presets.
  \item Hand-tuning materials is time-consuming, subjective, and often produces \emph{visually plausible yet physically incorrect} assets that break downstream FEM or game-physics pipelines.
  \item A method that automatically maps arbitrary 3D objects: triangle meshes, signed-distance fields (SDFs), Gaussian splats, or voxel grids to \emph{simulation-ready, per-voxel material fields} would allow rapidly simulating objects without handcrafting.
  \end{itemize}

\item \textbf{Problem Statement}
  \begin{itemize}
  \item \emph{Ill-posed inverse problem}: given only shape (and possibly texture), infer internal material parameters that are not directly observable.
  \item \emph{Data scarcity and heterogeneity}: real FEM datasets with ground-truth $E,\nu,\rho$ are rare; existing simulators store properties in incompatible units and coordinate frames.
  \item \emph{Current practice}:
    \begin{itemize}
    \item Manual label transfer or look-up tables based on coarse "wood/metal/plastic" classes.
    \item Vision-based methods predict surface appearance rather than bulk mechanics, and do not guarantee \emph{thermodynamic feasibility} or smooth interpolation in the material space.
    \end{itemize}
  \item \textbf{Specific gap}: no prior work produces \emph{volumetric} material fields that (i) generalise across 3D representations, (ii) respect physical constraints, and (iii) are differentiable for gradient-based downstream tasks.
  \end{itemize}

\item \textbf{Proposed Approach (high-level)}
  \begin{itemize}
  \item \textbf{Representation-agnostic voxelisation} converts input meshes, SDFs, or Gaussian splats into a unified occupancy grid at training time; at inference, voxelisation is computed on-the-fly.
  \item \textbf{Geometry-aware appearance features}: render multiple object views; extract DINO-v2 features per rendered images; back-project to voxels to obtain \emph{visual features}.
  \item \textbf{3D VAE for material inference}
    \begin{itemize}
    \item Transfrmer encoder-decoder that produces a 2D latent which is run through the material triplet vae decoder.
    \item The triplet vae takes this latents and produces material triplet composed on $E, \nu, \rho$.
    \end{itemize}
  \item Embedding each voxel in the \emph{learned manifold} of valid materials guarantees that interpolations (e.g., during style transfer or shape morphing) remain physically plausible.
  \item Using DINO features to learn visual details makes the methods very generalizable and easily extendable.
  \item Triplet-VAE decouples material validity from geometry.
\end{itemize}

\item \textbf{Impact \& Applications}
  \begin{itemize}
  \item \emph{Digital twins}: fast generation of thousands of materialised variants for environments.
  \item \emph{Robotics simulation}: realistic simulation of environments and robots without per-object calibration.
  \item Broader vision: bridges the gap between asset generation models or asset generation tools and simulation stacks, paving the way toward fully automated \emph{sim-ready asset pipelines}.
  \end{itemize}

\item \textbf{Contributions}
  \begin{itemize}
  \item First end-to-end framework that converts arbitrary 3D assets into \emph{simulation-ready volumetric material fields} without manual authoring.
  \item A \emph{Material-Triplet-VAE} with flow posterior that guarantees physically feasible $E,\nu,\rho$ and permits latent arithmetic for material interpolation/extrapolation.
  \item Extensive evaluation through high-fidelity FEM simulation demonstrating accurate stress–strain prediction and superior generalisation across meshes, SDFs, and Gaussian splats.
  \end{itemize}
\end{itemize}

\section{Related Works}

Clearly state that the closest work to us is SOPHY. However, we have a few benefits to it:
\begin{itemize}
    \item Our approach can be considered similar to us is SOPHY however we qualitatively compare and contrast with SOPHY due to absence of both code and data.
    \item we have fine-grained material values, example not just plastic but different values inside the humongous range of plastic
    \item we do any geometry not just point clouds
    \item we do volumetric properties not surface properties
    \item we easily handle >2-3 properties per object, clearly state that this point is derived only from the publicly released demos of the work but we aren't able to verify this due to absence of code and data
\end{itemize}

Other related work:

\begin{itemize}
    \item Start by clearly stating our setting, we need an object in (almost-) any representation and then predict \emph{spatially-varying volumetric} properties.
    \begin{itemize}
        \item {\color{red}detailed related work is at: \href{https://docs.google.com/spreadsheets/d/1MATEuqKsKqOJJWd4cPpjR5fgq4oMWdmkdM0lyhTwMMQ/edit?usp=sharing}{Google Doc}}
        \item We stress that our approach is different and cannot be compared with video-based methods unlike PhysDreamer, PAC-NeRF, DANO, PIE-NeRF, Phy124, and SDS-based methods. These methods often require dynamic frames like 4D Gaussian Dataset or complete multiview videos.
        \item More recent datasets, including ABO, Matsynth, and BlenderVault, incorporate surface texture information for each model. However be very careful, these are materials for \emph{photorealistic rendering}, not physical materials.
        \item Datasets such as ShapeNet-Mat, 3DCoMPaT, 3DCoMPaT200, and 3DCoMPaT++. These are (1) very small, smaller than our dataset (2) highly unreliable, these do have part-level material labels their annotations are very coarse and usually have highly coarse material names, and (3) the objects themselves are not high quality unlike simready objects which is probably the highest possible quality: perfect meshes and manually annotated fien parts. \masha{Also seems like ABO (Amazon Berkeley Objects) was used to benchmark density/mass estimation by PUGs and maybe Nerf2Physics. Can any other datasets be used for eval, whether image-based or 3D?}
        \item Many papers have claimed doing this in the context of pure 4D reconstruction and 4D generation, however this is a completely seperate even from an application perspective.
        \item One could still consider dynamic 3D reconstruction and dynamic 3D generation somewhat similar from an application perspective but the main part is we can do \emph{physically-ground novel interactions}.
        \item These collectively justify the gap we claimed in the literature even after the very recent works.
    \end{itemize}
\end{itemize}

\section{Method}

\masha{This is too much for one section. At least, the data annotation should be a separate section. Let's write up the various parts and then it will be clearer what should be split off. You essentially have 3 parts: 1) materials latent space (data and learning the material VAE, 2) generating training data with VLM, 3) graining 3D VAE. You can't quite go in that order, as you need an overview at some point of how all these things fit together, and it's good to have that overview at the start.} 

\subsection{Data Creation}

\begin{itemize}
    \item We start with repositories of high resolution part segented 3D meshes: simready, residential, commercial, and vegetation.
    \item We also have part-wise english material names for each part, semantic usage of each part, name of the object and name of parts, sometimes density, and categorization.
    \item Retrieve closest materials from material names.
    \item Use rendered objects, textures, and aforemention information to refine material property estimates with a vlm.
\end{itemize}

\subsection{Material VAE}

\begin{itemize}
    \item We train a 2-dimensional VAE to generate material triplets.
    \item With standard VAE tricks.
\end{itemize}

\subsection{3D VAE}

\begin{itemize}
    \item We render the object from multiple views and get 2D image features for all the views.
    \item We voxelize the object and propogate the 2d image features for all the voxels.
    \item The TRansformer encoder-decoder is trained to predict material properties for each voxel with a regression-style loss.
\end{itemize}

\section{Experiments}

\masha{Let's organize in to all the usual sections: Datasets \& Mertrics, Baselines, Experimental Setup, Results. What would you like to include for the Material VAE eval?}
Qunatitative:

\begin{itemize}
    \item We first show we can recover material values.
    \begin{itemize}
        \item From our high-quality dataset we made a \emph{hold-out} teste dataset of 200 objects.
        \item We scan {\color{red}x} objects and train splats on them and manually annotate ground truth properties.
        \item We then measure standard metrics: MSE distance, relative errors as well as material specific metrics: density-normalized counterparts, ashby indices, shear modulus, bulk modulus, bray-curtis, and composite ratio.
        \item In supplementary we provide experiments to demonstrate how standard metrics relate to simulation metrics.
    \end{itemize}
    \item We then report volume-change erros and potential-energy change erors on:
    \begin{itemize}
        \item predicted materials and ground truth materials on cubes
        \item on actual objects (less conclusive)
    \end{itemize}
\end{itemize}

Qualitative:

\begin{itemize}
    \item Focus a lot on this because the quantitative metrics are a bit harder to truly appreciate opposed to usual metrics like ROGUE, or accuracy, or any good VRs.
    \item Simulate a small set of objects and do a user study.
    \item Demonstrate differences in simulation when compared with a segmentation tool + LLM baseline particularly on objects like vegetation, and deformables.
\end{itemize}

\section{Discussion and Limitations}

\begin{itemize}
\item \textbf{Concise recap of what we did}
  \begin{itemize}
  \item Proposed a representation-agnostic pipeline that maps any 3D asset (mesh/SDF/GS/voxel) to a \emph{volumetric field of physically valid material triplets} $(E,\nu,\rho)$.
  \item Introduced the \emph{Material-Triplet-VAE} whose learned latent space generates feasible materials, supports smooth interpolation, and decouples material validity from geometry.
  \item Demonstrated xxx while requiring \emph{zero} manual authoring.
  \end{itemize}

\item \textbf{Why this matters}
  \begin{itemize}
  \item Bridges the long-standing gap between geometry-centric asset libraries and physics-centric simulation engines; assets become \emph{"drag-and-drop sim-ready."}
  \item Allows doing self-updating digital twins where scanned objects are endowed with physically plausible interiors on-the-fly. Allows doing robot learning in any environment.
  \end{itemize}
\end{itemize}

\subsection{Limitations}

\begin{itemize}
\item \textbf{Data scarcity \& label noise}
  \begin{itemize}
  \item Supervision still relies on scarce, sometimes \emph{expert-tweaked} material tables; rare composites are under-represented, leading to biased predictions in those regimes.
  \item VLM-refined labels improve consistency but occasionally propagate \emph{textural bias}.
  \end{itemize}

\item \textbf{Model assumptions}
  \begin{itemize}
  \item We voxelise at a fixed resolution; some aspects of the material may be oversmoothed, causing stiffness underestimation.
  \end{itemize}

\item \textbf{Scalability \& performance}
  \begin{itemize}
  \item Memory footprint grows cubically with resolution.
  \end{itemize}
\end{itemize}

\subsection{Future Work}

\begin{itemize}
\item \textbf{Richer physics}
  \begin{itemize}
  \item Extend triplet to a \emph{septet} $(E,\nu,\rho,\sigma_y,G,\alpha_T,c_p)$ capturing yield strength, shear modulus, thermal expansion, and specific heat; retrain with a hierarchical VAE to keep sampling tractable.
  \item Train adapater newtworks to take our real physics materials into simulator specific materials like take our real physics materials and train a network to convert them into a SPH material.
  \end{itemize}

\item \textbf{Adaptive \& multi-resolution geometry}
  \begin{itemize}
  \item Replace uniform voxels with \emph{octree} or \emph{implicit neural fields} to preserve thin shells while keeping memory linear in surface area.
  \end{itemize}

\item \textbf{Data augmentation \& semi-supervision}
  \begin{itemize}
  \item Leverage differentiable simulators to generate synthetic stress–strain curves for under-represented materials, using \emph{self-consistency losses} to refine noisy labels.
  \item Explore \emph{contrastive cross-modal pre-training} where tactile or audio impact data anchors material embeddings.
  \end{itemize}

\item \textbf{Broader horizons}
  \begin{itemize}
  \item Apply the learned material manifold to \emph{inverse design}: optimise geometry and material jointly.
  \end{itemize}
\end{itemize}

\section{Conclusion}

\begin{itemize}
    \item This work demonstrates a way to couple geometric representations with volumetric, physically valid material parameters through a common latent space. By automating the inference of elastic moduli, Poisson ratios, and densities at voxel resolution, it removes the manual lookup tables and ad-hoc presets that currently separate asset creation from simulation pipelines.
    \item Treating material assignment as a learned, differentiable mapping makes it straightforward to integrate structural optimisation, uncertainty estimation, and large-scale data generation within a single workflow.
\end{itemize}
